Actively Discovering New Slots for Task-oriented Conversation

Existing task-oriented conversational search systems heavily rely on domain ontologies with pre-defined slots and candidate value sets. In practical applications, these prerequisites are hard to meet, due to the emerging new user requirements and ever-changing scenarios. To mitigate these issues for better interaction performance, there are efforts working towards detecting out-of-vocabulary values or discovering new slots under unsupervised or semi-supervised learning paradigm. However, overemphasizing on the conversation data patterns alone induces these methods to yield noisy and arbitrary slot results. To facilitate the pragmatic utility, real-world systems tend to provide a stringent amount of human labelling quota, which offers an authoritative way to obtain accurate and meaningful slot assignments. Nonetheless, it also brings forward the high requirement of utilizing such quota efficiently. Hence, we formulate a general new slot discovery task in an information extraction fashion and incorporate it into an active learning framework to realize human-in-the-loop learning. Specifically, we leverage existing language tools to extract value candidates where the corresponding labels are further leveraged as weak supervision signals. Based on these, we propose a bi-criteria selection scheme which incorporates two major strategies, namely, uncertainty-based sampling and diversity-based sampling to efficiently identify terms of interest. We conduct extensive experiments on several public datasets and compare with a bunch of competitive baselines to demonstrate the effectiveness of our method. We have made the code and data used in this paper publicly available.

==> data.tex <==
\section{NTD Dataset}
Since there are no existing NTD datasets, we collect a new large-scale one to demonstrate the feasibility of the NTD task and support model developments. We first elaborate on the data construction and processing in detail, then display the statistics of the collected dataset and perform analysis.

\subsection{Data Collection}
The dataset is collected by enabling conversations between human-to-human role-playing pairs under travel scenarios. To support this, we first build a crowd-sourced knowledge base $\mathcal{K}$ from Foursquare City Guide about a famous tourist city on five domains: food, hotel, nightlife, sightseeing and shopping mall. There are 1,771 venues with detailed information fields included in $\mathcal{K}$ as shown in Table \ref{tab:domain}. We then crawl reviews and forum threads from \url{tripadvisor.com} and \url{lonelyplanet.com} to construct real user settings. It provides detailed venue goals $\mathcal{G}$ with structured preferences for user as guidelines to help regularizing the conversation flow while allow expression flexibility. Given search base $\mathcal{K}$ and user goals $\mathcal{G}$, we build an online platform to support conversation collection, where human-to-human pairs are formed to find certain venues. The user role-plays a traveler under an specific user setting sampled from $\mathcal{G}$. An target venue(s) information is provided but the user cannot expose unique information such as name, address or telephone number. The agent player observes the whole venue database $\mathcal{K}$ to find venues, provide recommendations and complete tasks such as `get address' or `check reservation'. We provided them with search engines. A total of 87 undergraduate students are recruited in the data collection process. More details can be found in Appendix \ref{A}.

\begin{table}[!htp]
	\centering
	\small
	\setlength\tabcolsep{4pt}
	\caption{\label{tab:domain}
		Venue distribution over different domains.}\vspace{-0.2cm}
	\begin{tabular}{ l|ccccc}
		\hline\xrowht[()]{4pt}
	    & \textbf{food}&\textbf{hotel} &\textbf{nightlife}& \textbf{mall} &\textbf{sight}\\
		\hline\xrowht[()]{4pt}
		\textbf{Venue}&1,162&83&128&96&302\\
		\hline\xrowht[()]{4pt}
		\textbf{Review} &27,303&2,661&3,064&3,803&6,019\\
		\hline\xrowht[()]{4pt}
		\multirow{6}{*}{\textbf{Fields}} & \multicolumn{5}{l}{drinks / music / reservations / dining options /}\\
		& \multicolumn{5}{l}{stores / wifi / menus / outdoor seating / review /} \\
		& \multicolumn{5}{l}{venue domain / venue neighborhood / smoking / }\\
		& \multicolumn{5}{l}{wheelchair accessible / parking / venue score /}\\
		& \multicolumn{5}{l}{restroom / credit cards / pricerange / telephone /} \\
		& \multicolumn{5}{l}{venuename / venue address} \\
		\hline
	\end{tabular}
	\vspace{-0.3cm}
\end{table}


\subsection{Annotation and Quality Control}
To ensure the quality of conversation data collected, we apply a five-step scheme of training, collection, checking, modification, and re-checking in sequence. Before collection, we carry out training for all participants for about half an hour. When dialogues are generated, a manual quality checking sifts out those unqualified ones and the participants will be notified to modify further. A second check would be applied and unqualified ones will be rejected with no pay. 

Our annotation of novel terms (NTs) is also divided into three stages: collection, modification and manual correction. During collection, the user players are asked to select out important information or salient terms, which are the target terms we want to find. Next, the generated dialogue with annotations will be manually checked and unqualified ones will be modified by their original generator. After that, we further do manual correction to eliminate some typos and errors. We estimate the inter-annotator agreement for the last stage results by calculating the averaged kappa value \cite{fleiss1971measuring} for all dialogue acts over 300 random sampled turns. The high score of $\kappa = 0.82$ demonstrates good agreements.

\subsection{Data Analysis}
Table \ref{tab:data} shows the general statistics of the conversation dataset \footnote{The dataset and code have been submitted together. We will make them public if got accepted.}. We finally collected \zznote{collect} $5,106$ successful conversations where all venues in goal are found by the agent and tasks are completed \footnote{We delete dialogues that failed to find the correct venue(s). Sensitive information is also removed.}. The average turn number is $7.8$ which indicates rich contextual information to be modeled. In general, we have dialogues in five domains, where we have  $808$ single-domain dialogues and $4,298$ multi-domain dialogues. Note that we created $386$ goals, and dialogue collected under the same goal might be relatively similar to each other. Hence, to emphasize on the novel term situation, we randomly split our dataset into \textit{training/testing/validation} sets based on different goals.
\begin{table}[t]
	\centering
	\caption{\label{tab:data}
		The general statistics of the conversation data.}
	\begin{tabular}{ll}
		\hline
		\textbf{Entry} & \textbf{Number}\\
		\hline
		\# dialogues &  5,106 \\
		\# turns & 39,759 \\ 
		\# domains & 5\\
		\# goals & 386\\
		\# total venues in DB & 1,771\\
		\# total reviews in DB & 42,850\\
		\hline
	\end{tabular}
\vspace{-0.3cm}
\end{table}

\begin{figure}[!htp]
	\centering
	\vspace{-0.1cm}
	\subfigure[Consensus]{\includegraphics[width=0.48\linewidth]{img/consensus_2.png}}
	\hspace{1mm}
	\subfigure[POS constitution]{\includegraphics[width=0.48\linewidth]{img/constitution.pdf}}
	\vspace{-0.1cm}
	\caption{(a) Consensus check via the T-SNE algorithm \zznote{add reference}.  We show conversations of 20 randomly selected goals. (b) The POS constitution of the selected terms.}
	\vspace{-0.3cm}
	\label{consensus}
\end{figure}

To test whether these user selected terms are valid or not, we further conduct a consensus check. As shown in Figure \ref{consensus} (a), we visually assess the consensus by showing the dialogue representation clustering effects. We randomly select 20 goals, use the user selected terms to represent the dialogues under these goals into a sequence, and encode the sequence with BERT to get the CLS position vector. We cluster such representation of dialogue in the selected set into 20 clusters, and then projecting them with t-SNE \cite{van2008visualizing}. Through inspecting these formed clusters, we find that users tend to select similar critical terms in dialogues under the same goal. Also, the terms selected in dialogues under different goals are relatively diverse.

We also analyze the user selected terms regarding its POS construction. The result is shown in Figure \ref{consensus} (b). The ordering of the POS tags starts towards the center and
radiates outwards. The arc length is proportional to the number of words containing the POS tag. It indicates that most terms start with \textit{noun} or \textit{adj.} 

